Teaching Concurrent Software Design: A Case Study Using Android

In this article, we explore various parallel and distributed computing topics from a user-centric software engineering perspective. Specifically, in the context of mobile application development, we study the basic building blocks of interactive applications in the form of events, timers, and asynchronous activities, along with related software modeling, architecture, and design topics.

==> Acknowledgement/acknowledgement.tex <==
\fchapter{ACKNOWLEDGEMENTS}
\pagestyle{myheadings}
%%%%%%%%%%CHANGE HERE%%%%%%%%%%
Acknowledgements go here.

==> Title/title.tex <==
\pagestyle{empty}
\begin{center}
%%%%%%%%%%CHANGE HERE%%%%%%%%%%
CDER Book\\
%\vspace{1.7in}
%by\\
%\vspace{1.7in}
%%%%%%%%%%CHANGE HERE%%%%%%%%%%
%FIRST AUTHOR\\
%SECOND AUTHOR\\

\vspace{2in}
%%%%%%%%%%CHANGE HERE%%%%%%%%%%
NSF/IEEE-TCPP CDER Curriculum Initiative on Parallel and Distributed Computing \\
\vspace{.2in}
%%%%%%%%%%CHANGE HERE%%%%%%%%%%
2013
\end{center}


